A new source for light dark matter isocurvature in low scale inflation

Light scalar and pseudoscalar particles are compelling dark matter candidates, with a vast running experimental program to discover them. Previous studies have shown that these light fields can generate sizable isocurvature perturbations in high scale inflationary models. Thereby, dark matter existence and cosmic microwave background measurements impose an upper bound on the inflationary scale. In this work, focusing on the axion case, we point out that light fields present during inflation can generate important isocurvature perturbations also in scenarios of low-scale inflation. In our mechanism, the axion field starts with some non-zero field value during inflation and rolls along its potential. Since inflation has a different duration in different patches of the universe, different regions will then have different values of the axion field, generating cold dark matter isocurvature modes. These modes are fully correlated with the adiabatic ones and share the same spectral index. In this scenario, the axion mass determines a lower bound on the Hubble parameter during inflation.

==> OldStuff.tex <==
\textbf{Old stuff follows}
 
We can find therefore that

\begin{equation}
\frac{\delta a_{l}}{\dot{a}_{l}}(t)  =\frac{C_{1}(\mathbf{k})}{H}-2 C_{3}(\mathbf{k}) \frac{H V_{inf}}{V_{inf}+V_{a}} 
\label{Eq:Iso_Adia}
\end{equation}

Where $C_1$ is the adiabatic mode, and $C_3$ is the isocurvature mode given by 
\begin{equation}
C_3 = d_a - d_{inf} \approx -d_{inf},
\end{equation}

where we have explicitly assumed that $V^{\prime}_{\inf}<V^{\prime}_a$, which is the case for the our low scale inflationary scenario where $H\gtrsim m_a$. This can be seen by looking at:
\begin{eqnarray}
    V^{\prime}_{\inf}&\sim& H \dot{\phi} \sim 10^{-5} H^3 \sim 10^{-5} m_a^3\nonumber\\
    V^{\prime}_a &\sim& m^2_a f \theta_{QCD} 
\end{eqnarray}

Where $\theta_{QCD} \sim  \sqrt{\frac{10^{12}~GeV}{f}} > 10^{-3}$. With this, we can finally calculate using [Lesgourgues et al] 

\begin{equation}
    S_{\alpha} = 4\left<\left|\frac{\delta a}{a}\right|^2 \right> = 4 \left<\left|\frac{\delta a}{\dot{a}}\right|^2 \right> \left(\frac{\dot{a}}{a} \right)^2
\end{equation}

Using Eq.~\ref{Eq:Iso_Adia} 

\begin{equation}
     \Delta^2_S= 8 {\bf C}^2_3 H^2 \left(\frac{\dot{a}}{a}\right)^2  \equiv 4 {\bf C}_1^2 H^2\left(\frac{\dot{a}}{a}\right)^2 = 4\Delta^2_R \left(\frac{1}{a} \frac{da}{dN}\right)^2
\end{equation}

Using this, we find that 
\begin{equation}
\label{eq:iso_bound}
\alpha \equiv f_{\iso}^2\equiv \frac{ \Delta^2_S}{ \Delta^2_S+  \Delta^2_R} \approx 4 \left(\frac{1}{a} \frac{da}{dN}\right)^2
\end{equation}

\textit{QCD Axion Isocurvature from low scale inflation} -- For the QCD axion, we take the assumption that the QCD axion makes up all of the DM abundance. For the QCD axion, $\theta_{QCD} \sim  \sqrt{\frac{10^{12}~GeV}{f}}$, and the potential is \cite{GrillidiCortona:2015jxo}
\begin{equation}
    V(a)= -m_{\pi}^2f_{\pi}^2\sqrt{1-\frac{4 m_u m_d}{\left(m_u+m_d\right)^2} sin^2\frac{a}{2f_a}}
\end{equation}
In our ballpark parameter space, the scale of inflation is in the GeV to TeV range, for which the minimal length of inflation is around 30 e-folds. 

We solve the equation of motion $3H\dot{a} = V'(a)$, and set the condition that $a(t_{end}) =\theta_{QCD}$. We solve the EOMs and set a bound using $f_{iso}>0.1$(Planck), and by taking evaluating $\left(\frac{1}{a} \frac{da}{dN}\right)$ (Eq.~\ref{eq:iso_bound}) 30 e-folds before the end of inflation. The corresponding bound is fitted well by  
\begin{eqnarray}
\Lambda_{inf}&>&280\,\mathrm{GeV} \sqrt{\frac{10^{12}\,\mathrm{ GeV}}{f_a}}\nonumber\\ 10^{12}\,\mathrm{GeV} &\lesssim& f_a \lesssim 6\times10^{17}\,\mathrm{GeV}
\end{eqnarray}
where 

Where for $f_a$ far below $10^{12}$ the relic abundance is not reproduced and for $f_a$ above $6\times10^{17}$ the isocurvature production is suppressed (will find out why). 

The projected bound for CMB-S4 together with SKA(?) is $f_{iso}>0.01$, which would imply 
\begin{eqnarray}
\Lambda_{inf}&>&500\,\mathrm{GeV} \sqrt{\frac{10^{12}\,\mathrm{ GeV}}{f_a}}\nonumber\\ 10^{12}\,\mathrm{GeV} &\lesssim& f_a \lesssim m_{Pl}
\end{eqnarray}
Here there is no upper bound on $f_a$ below $m_{Pl}$

%I'm thinking we can just leave it with the actual bound, since this is not what our paper is about
With this we derive a condition for the axion to be all of DM. We derive the bound by assuming that the axion must start at least $H/2\pi$ away from the top of its potential, 30 e-folds before the end of inflation. This is effectively the farthest away from the minimum that the axion can be at that point, and therefore this will generate the neccessary condition. We therefore solve the axion slow roll EOM during inflation, with the condition that 
\begin{equation}
    \frac{a\left(t_{end}\right)}{f_a}\approx \sqrt{\frac{10^{12}\,\mathrm{ GeV}}{f_a}}
\end{equation}

%A second approach can be taken by assuming that the initial condition is not too tuned, i.e. $\theta_0 \sim {\cal O}(1)$, which we take to be a few hundred e-folds before the end of the inflation to also not have a tuned period of inflation. 

This condition is solved for numerically and we find that requiring that $a\left(t_{end}-\frac{30}{H}\right)<\pi f_a-\frac{H}{2\pi}$ corresdponds to

\begin{equation}
\Lambda_{\rm inf} > 264\,\mathrm{GeV} \left(\frac{10^{12}\,\mathrm{ GeV}}{f_a}\right)^{0.53}
\end{equation}

We see that the current isocurvature bound is very close to the relic abundance constraint, and therefore currently doesn't offer much more new information. However, new experiments may probe a scale of inflation not currently constrained by the relic abundance constraint. This also makes a new discovery of a CDM isocuravture component in the primordial spectrum which is fully correlated with the adiabatic one possible within the realm of axion DM. 

For a general ALP model, we take a simple cosine potential, with free parameters $f_a$ and $m_a$. We require that the relic abundance is fitted, which is given by
\begin{equation}
    a\left(t_{end}\right)^2 \sim \mathrm{eV} \frac{m_{Pl}^{3 / 2}}{m_a^{1 / 2}}
\end{equation}
From solving the EOM, we can again find $\left(\frac{1}{a} \frac{da}{dN}\right)$ (Eq.~\ref{eq:iso_bound}) 30 e-folds before the end of inflation. 

We once again solve numerically and then fit the results as
\begin{equation}
    \Lambda_{inf}\gtrsim\sqrt{m_a m_{Pl}} \left\{\begin{array}{c c}2.5& f_{iso}<0.1 \\ 4.5& f_{iso}<0.01\end{array}\right. 
\end{equation}

This bound is found to be valid for  
\begin{equation}
  f\gtrsim  \left(\frac{1\,\mathrm{eV}}{m_a}\right)^{\frac{1}{4}}\left\{\begin{array}{c c}2ֿ\times10^{12}& f_{iso}<0.1 \\ 8\times 10^{10}& f_{iso}<0.01\end{array}\right. 
\end{equation}
